The devil is in the tails: the role of globular cluster mass evolution on stream properties

We present a study of the effects of collisional dynamics on the formation and detectability of cold tidal streams. A semi-analytical model for the evolution of the stellar mass function was implemented and coupled to a fast stellar stream simulation code, as well as the synthetic cluster evolution code EMACSS for the mass evolution as a function of a globular cluster orbit. We find that the increase in the average mass of the escaping stars for clusters close to dissolution has a major effect on the observable stream surface density. As an example, we show that Palomar 5 would have undetectable streams (in an SDSS-like survey) if it was currently three times more massive, despite the fact that a more massive cluster loses stars at a higher rate. This bias due to the preferential escape of low-mass stars is an alternative explanation for the absence of tails near massive clusters, than a dark matter halo associated with the cluster. We explore the orbits of a large sample of Milky Way globular clusters and derive their initial masses and remaining mass fraction. Using properties of known tidal tails we explore regions of parameter space that favour the detectability of a stream. A list of high probability candidates is discussed

==> mf_evolve.tex <==


In this section we present an algorithm to numerically evolve the stellar mass
function (MF). Various prescriptions for the time-dependent MF exist
\citep[e.g.][]{2009A&A...507.1409K,2013MNRAS.433.1378L}. We aim to develop a
prescription that can be coupled to the fast cluster code \emacss. Because
\emacss\ solves a set of coupled ODEs, we develop a prescription for the rate of
change of the number of stars and stellar remnants  as a function of stellar
mass $m$. We aim to correctly describe the preferential ejection of low-mass
stars as the result of two-body relaxation, and the formation of stellar
remnants as the result of stellar evolution. Below we describe the algorithm.

To evolve the MF of  stars and remnants, we define $\nbin\simeq100$
logarithmically spaced mass bins between $0.1\,\msun$ and $100\,\msun$. At $t=0$
the number of stars in each bin, $\nj$, is found from the stellar initial mass
function (IMF, $\dr N/\dr\mi$), the total number of stars in the cluster $N$ and
the width of the individual bins $\Delta \mj$ as

\begin{equation}
\nj= N \left.\frac{\dr N}{\dr\mi}\right|_{m_j} \Delta \mj
\end{equation}
such that $\sum_{j=1}^{\nbin} \nj = N$ and $\sum_{j=1}^{\nbin} \nj\mj = M_{\rm
i}$, where $M_{\rm i}$ is the initial mass of the cluster. We then consider that
$\nj = \njs  + \njr$, with $\njs$ the number of stars and $\njr$ the number of
remnants as a function of mass. At $t=0$ there are no remnants. 

We then evolve $\njs$ and $\njr$ with an ODE solver and expressions for the rate
of change of $\njdot = \njsdot + \njrdot$. Both stellar evolution and escape of
stars contribute to these rates, which we discuss in the next sections. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stellar evolution}
\label{ssec:sev}
To  evolve stars by stellar evolution, we move stars that reach the end their
main sequence life from $\njs$ to $\njr$.  We approximate  the main-sequence
lifetimes by

\begin{equation}
\tms(\mi) = 0.21\exp\left(10.4\mi^{-0.322}\right),
\label{eq:tms}
\end{equation}
which describes the main sequence life times of stars $0.5<\mi/\msun<30\,\msun$
and $\feh=-0.5$ to within 10\% compared to the SSE (Single-Star Evolution)
models of \citet{2000MNRAS.315..543H}, \comm{which provides a set of analytic
    relations that approximate the evolution of stars of different masses and
chemical composition}. \comm{In our MF evolution method} stars are assumed to
have a constant mass $\mi$ until $\tms(\mi)$ is reached and then their mass is
reduced by a factor

\begin{align}
\fifm=
\begin{cases}
0 & \mi>10\,\msun,\\
0.56(\mi/\msun)^{-0.56} & \mi\le10\,\msun.
\end{cases}
\end{align}

Removing all stars with $\mi>10\,\msun$ corresponds to 0\% retention of black
holes. A single relation for the masses of neutron stars and white dwarfs
reproduces the results from SSE to within 10\%. The most massive neutron stars
is $1.54\,\msun$ and a solar mass star results in a $0.56\,\msun$ white dwarf.

\comm{We introduce stellar evolution by removing stars are at a rate}
\begin{align}
\njssevdot  = 
\begin{cases}
    \njs\left(\dfrac{t-\tmsright}{\sigmat}\right), &t>\tmsright,\\
0,& t<\tmsright,
\end{cases}
\end{align}
where $\tmsright$ is the main sequence life time of a star with $m_j + 0.5\Delta
m_j$ (i.e. corresponding to the right side of  bin $j$) and $\sigmat$ sets the
speed with which the bin is emptied. From experiments we find smooth evolution
of the mass function when using $\sigmat = 0.7(\tmsright-\tmsleft)$, where
$\tmsleft = \tms(m_j-0.5\Delta m_j)$ i.e. the life time of a star with mass
corresponding to the left side of bin  $j$.

While stars are being removed, remnants are being create, hence we fill bins of
the remnants mass function at a rate

\begin{align}
\nkrdot(\mto(t)\fifm)&=- \njssevdot,
\end{align}
where $\mto(t)$ is the turn-off mass at time $t$, which is found form the
inverse of the main sequence time relation (equation~\ref{eq:tms}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Escape}
In the pre-collapse phase we assume that the escape rate is independent of
stellar mass, i.e. $\njsdot = \njs \dot{N}/N$ (similarly for $\njrdot$), where
$\dot{N}$ is the total escape rate of the cluster which comes from {\sc emacss}.
After core collapse (also given by {\sc emacss}) we apply an escape rate to each
bin

\begin{align}
\njescdot  = \dot{N} \frac{\njs + \njr}{N} \frac{g(m_j)}{\sum_j g(m_j)}
\end{align}
where

\begin{align}
g(m_j)  = 
\begin{cases}
\left(m_j/\md\right)^{1/2} - 1, &m_j<\md,\\
1,                              &m_j\ge \md.
\end{cases}
\end{align}

This simple functional form for $\njescdot$ was found by matching the time
derivatives of the functional forms for the MF as a function of time given by
\cite{2013MNRAS.433.1378L}. With a value of $\md\simeq1.1\,\msun$ we find a good
agreement with results from $N$-body models (see example in Fig.~\ref{fig1}).
The 100\% retention of stars and remnants more massive than $\md$ is only
becoming problematic when less than a few \% of the initial mass is remaining,
and hence this approximation is good enough for our purpose. The escape rate is
divided over the stars and remnants as $\njsescdot = \njescdot \njs/\nj$
(similarly for $\njrescdot$), such that $\njescdot = \njsescdot + \njrescdot$.



